A Peek into Token Bias: Large Language Models Are Not Yet Genuine Reasoners

This study introduces a hypothesis-testing framework to assess whether large language models (LLMs) possess genuine reasoning abilities or primarily depend on token bias. We go beyond evaluating LLMs on accuracy; rather, we aim to investigate their token bias in solving logical reasoning tasks. Specifically, we develop carefully controlled synthetic datasets, featuring conjunction fallacy and syllogistic problems. Our framework outlines a list of hypotheses where token biases are readily identifiable, with all null hypotheses assuming genuine reasoning capabilities of LLMs. The findings in this study suggest, with statistical guarantee, that most LLMs still struggle with logical reasoning. While they may perform well on classic problems, their success largely depends on recognizing superficial patterns with strong token bias, thereby raising concerns about their actual reasoning and generalization abilities. Codes and data are open-sourced at https://github.com/bowen-upenn/llm_token_bias.

==> figures/hypothesis1.1_claude-3-opus-20240229.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &             0.16  \\
  1 & zs\_cot             & linda\_original            &             0.48  \\
  2 & baseline           & linda\_variant\_four        &             0.43  \\
  3 & zs\_cot             & linda\_variant\_four        &             0.47  \\
  4 & baseline           & linda\_variant\_one\_because &             0.34  \\
  5 & zs\_cot             & linda\_variant\_one\_because &             0.32  \\
  6 & baseline           & linda\_variant\_one\_sothat  &             0.18  \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &             0.06  \\
  8 & baseline           & linda\_variant\_one\_to      &             0.53  \\
  9 & zs\_cot             & linda\_variant\_one\_to      &             0.46  \\
 10 & baseline           & linda\_variant\_three       &             0.33  \\
 11 & zs\_cot             & linda\_variant\_three       &             0.53  \\
 12 & baseline           & sets\_original             &             0.715 \\
 13 & zs\_cot             & sets\_original             &             0.81  \\
 14 & baseline           & sets\_original\_framing     &             0.485 \\
 15 & zs\_cot             & sets\_original\_framing     &             0.495 \\
\hline
\end{tabular}

==> figures/hypothesis1.1_claude-3-sonnet-20240229.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &              0.11 \\
  1 & zs\_cot             & linda\_original            &              0.3  \\
  2 & baseline           & linda\_variant\_four        &              0.24 \\
  3 & zs\_cot             & linda\_variant\_four        &              0.51 \\
  4 & baseline           & linda\_variant\_one\_because &              0.15 \\
  5 & zs\_cot             & linda\_variant\_one\_because &              0.23 \\
  6 & baseline           & linda\_variant\_one\_sothat  &              0.26 \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &              0.43 \\
  8 & baseline           & linda\_variant\_one\_to      &              0.31 \\
  9 & zs\_cot             & linda\_variant\_one\_to      &              0.44 \\
 10 & baseline           & linda\_variant\_three       &              0.37 \\
 11 & zs\_cot             & linda\_variant\_three       &              0.39 \\
 12 & baseline           & sets\_original             &              0.04 \\
 13 & zs\_cot             & sets\_original             &              0.05 \\
 14 & baseline           & sets\_original\_framing     &              0.61 \\
 15 & zs\_cot             & sets\_original\_framing     &              0.78 \\
\hline
\end{tabular}

==> figures/hypothesis1.1_gpt-3.5-turbo.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &             0.05  \\
  1 & zs\_cot             & linda\_original            &             0.25  \\
  2 & baseline           & linda\_variant\_four        &             0.25  \\
  3 & zs\_cot             & linda\_variant\_four        &             0.48  \\
  4 & baseline           & linda\_variant\_one\_because &             0.62  \\
  5 & zs\_cot             & linda\_variant\_one\_because &             0.49  \\
  6 & baseline           & linda\_variant\_one\_sothat  &             0.76  \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &             0.57  \\
  8 & baseline           & linda\_variant\_one\_to      &             0.72  \\
  9 & zs\_cot             & linda\_variant\_one\_to      &             0.56  \\
 10 & baseline           & linda\_variant\_three       &             0.34  \\
 11 & zs\_cot             & linda\_variant\_three       &             0.44  \\
 12 & baseline           & sets\_original             &             0.275 \\
 13 & zs\_cot             & sets\_original             &             0.235 \\
 14 & baseline           & sets\_original\_framing     &             0.335 \\
 15 & zs\_cot             & sets\_original\_framing     &             0.465 \\
\hline
\end{tabular}

==> figures/hypothesis1.1_gpt-4-turbo.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &             0.57  \\
  1 & zs\_cot             & linda\_original            &             0.7   \\
  2 & baseline           & linda\_variant\_four        &             0.43  \\
  3 & zs\_cot             & linda\_variant\_four        &             0.53  \\
  4 & baseline           & linda\_variant\_one\_because &             0.14  \\
  5 & zs\_cot             & linda\_variant\_one\_because &             0.18  \\
  6 & baseline           & linda\_variant\_one\_sothat  &             0.23  \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &             0.35  \\
  8 & baseline           & linda\_variant\_one\_to      &             0.32  \\
  9 & zs\_cot             & linda\_variant\_one\_to      &             0.43  \\
 10 & baseline           & linda\_variant\_three       &             0.5   \\
 11 & zs\_cot             & linda\_variant\_three       &             0.47  \\
 12 & baseline           & sets\_original             &             0.995 \\
 13 & zs\_cot             & sets\_original             &             0.975 \\
 14 & baseline           & sets\_original\_framing     &             0.28  \\
 15 & zs\_cot             & sets\_original\_framing     &             0.275 \\
\hline
\end{tabular}

==> figures/hypothesis1.1_gpt-4o.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &             0.66  \\
  1 & zs\_cot             & linda\_original            &             1     \\
  2 & baseline           & linda\_variant\_four        &             0.61  \\
  3 & zs\_cot             & linda\_variant\_four        &             0.84  \\
  4 & baseline           & linda\_variant\_one\_because &             0.07  \\
  5 & zs\_cot             & linda\_variant\_one\_because &             0.25  \\
  6 & baseline           & linda\_variant\_one\_sothat  &             0.28  \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &             0.47  \\
  8 & baseline           & linda\_variant\_one\_to      &             0.33  \\
  9 & zs\_cot             & linda\_variant\_one\_to      &             0.46  \\
 10 & baseline           & linda\_variant\_three       &             0.57  \\
 11 & zs\_cot             & linda\_variant\_three       &             0.7   \\
 12 & baseline           & sets\_original             &             0.895 \\
 13 & zs\_cot             & sets\_original             &             0.915 \\
 14 & baseline           & sets\_original\_framing     &             0.16  \\
 15 & zs\_cot             & sets\_original\_framing     &             0.14  \\
\hline
\end{tabular}

==> figures/hypothesis1.1_llama-2-70b-chat.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &              0.1  \\
  1 & zs\_cot             & linda\_original            &              0.14 \\
  2 & baseline           & linda\_variant\_four        &              0.09 \\
  3 & zs\_cot             & linda\_variant\_four        &              0.11 \\
  4 & baseline           & linda\_variant\_one\_because &              0.32 \\
  5 & zs\_cot             & linda\_variant\_one\_because &              0.18 \\
  6 & baseline           & linda\_variant\_one\_sothat  &              0.46 \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &              0.27 \\
  8 & baseline           & linda\_variant\_one\_to      &              0.49 \\
  9 & zs\_cot             & linda\_variant\_one\_to      &              0.29 \\
 10 & baseline           & linda\_variant\_three       &              0.02 \\
 11 & zs\_cot             & linda\_variant\_three       &              0.04 \\
 12 & baseline           & sets\_original             &              0    \\
 13 & zs\_cot             & sets\_original             &              0    \\
 14 & baseline           & sets\_original\_framing     &              0    \\
 15 & zs\_cot             & sets\_original\_framing     &              0    \\
\hline
\end{tabular}

==> figures/hypothesis1.1_meta-llama-3-70b-instruct.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &             0.1   \\
  1 & zs\_cot             & linda\_original            &             0.25  \\
  2 & baseline           & linda\_variant\_four        &             0.08  \\
  3 & zs\_cot             & linda\_variant\_four        &             0.23  \\
  4 & baseline           & linda\_variant\_one\_because &             0.2   \\
  5 & zs\_cot             & linda\_variant\_one\_because &             0.23  \\
  6 & baseline           & linda\_variant\_one\_sothat  &             0.38  \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &             0.46  \\
  8 & baseline           & linda\_variant\_one\_to      &             0.41  \\
  9 & zs\_cot             & linda\_variant\_one\_to      &             0.42  \\
 10 & baseline           & linda\_variant\_three       &             0.46  \\
 11 & zs\_cot             & linda\_variant\_three       &             0.45  \\
 12 & baseline           & sets\_original             &             0.035 \\
 13 & zs\_cot             & sets\_original             &             0.085 \\
 14 & baseline           & sets\_original\_framing     &             0.05  \\
 15 & zs\_cot             & sets\_original\_framing     &             0.125 \\
\hline
\end{tabular}

==> figures/hypothesis1.1_meta-llama-3-8b-instruct.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &             0.38  \\
  1 & zs\_cot             & linda\_original            &             0.52  \\
  2 & baseline           & linda\_variant\_four        &             0.38  \\
  3 & zs\_cot             & linda\_variant\_four        &             0.28  \\
  4 & baseline           & linda\_variant\_one\_because &             0.28  \\
  5 & zs\_cot             & linda\_variant\_one\_because &             0.35  \\
  6 & baseline           & linda\_variant\_one\_sothat  &             0.47  \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &             0.48  \\
  8 & baseline           & linda\_variant\_one\_to      &             0.55  \\
  9 & zs\_cot             & linda\_variant\_one\_to      &             0.56  \\
 10 & baseline           & linda\_variant\_three       &             0.63  \\
 11 & zs\_cot             & linda\_variant\_three       &             0.48  \\
 12 & baseline           & sets\_original             &             0     \\
 13 & zs\_cot             & sets\_original             &             0.01  \\
 14 & baseline           & sets\_original\_framing     &             0.235 \\
 15 & zs\_cot             & sets\_original\_framing     &             0.265 \\
\hline
\end{tabular}

==> figures/hypothesis1.1_mistral-large-latest.tex <==
\begin{tabular}{rllr}
\hline
    & prompting\_method   & variant                   &   percent\_correct \\
\hline
  0 & baseline           & linda\_original            &             0.1   \\
  1 & zs\_cot             & linda\_original            &             0.35  \\
  2 & baseline           & linda\_variant\_four        &             0.09  \\
  3 & zs\_cot             & linda\_variant\_four        &             0.23  \\
  4 & baseline           & linda\_variant\_one\_because &             0.07  \\
  5 & zs\_cot             & linda\_variant\_one\_because &             0.1   \\
  6 & baseline           & linda\_variant\_one\_sothat  &             0.22  \\
  7 & zs\_cot             & linda\_variant\_one\_sothat  &             0.2   \\
  8 & baseline           & linda\_variant\_one\_to      &             0.28  \\
  9 & zs\_cot             & linda\_variant\_one\_to      &             0.3   \\
 10 & baseline           & linda\_variant\_three       &             0.32  \\
 11 & zs\_cot             & linda\_variant\_three       &             0.41  \\
 12 & baseline           & sets\_original             &             0.665 \\
 13 & zs\_cot             & sets\_original             &             0.66  \\
 14 & baseline           & sets\_original\_framing     &             0.095 \\
 15 & zs\_cot             & sets\_original\_framing     &             0.08  \\
\hline
\end{tabular}

==> sections/3_prelim.tex <==
\section{Preliminaries}\label{sec:prelim}
%\textbf{TODO: We shall make this section shorter.}
% \subsection{Logical Fallacies in Cognitive Science}
% \textbf{TODO: Add a prelim section to intro conjunction fallacy. The intro might be better to focus on token bias.}
In this work, we apply two kinds of logical fallacies discussed in the cognitive science literature\citet{tversky1983extensional, kahneman2011thinking}: conjunction fallacy and syllogistic fallacy to construct synthetic datasets on which we perform our token perturbation. In this section, we briefly discuss the reasoning logic of these problems. 
\paragraph{Conjunction Fallacy}
The most often-cited example of conjunction fallacy is called the Linda problem and framed as follows ~\citep{tversky1983extensional}:
\textit{Linda is 31 years old, single, outspoken, and very bright. She majored in philosophy. As a student, she was deeply concerned with issues of discrimination and social justice, and also participated in antinuclear demonstrations. Which is more probable?}
\begin{quote}
\vspace{-1mm}
\textit{(a) Linda is a bank teller.}\\
\textit{(b) Linda is a bank teller and is active in the feminist movement.}
\vspace{-1mm}
\end{quote}
\citet{tversky1983extensional} found that humans tend to prefer option (b). However, it is logically necessary that the probability of a conjunction of two events (e.g., Linda is a bank teller, {\it and} she is active in the feminist movement) is less than the probability of either event alone. 

\begin{comment}
\vspace{1mm}
\textit{Taylor Swift will embark on another tour in 2027. Which outcome do you think is more likely?}
\begin{quote}
\vspace{-1mm}
\textit{(a) Her first show is a flop.} \\
\textit{(b) Her first show is a flop but she will eventually sell over a million tickets for the entire tour.}
\vspace{-1mm}
\end{quote}

Commonly, both humans and LLMs might prefer option (b), reasoning that despite a potential initial setback, Taylor Swift's consistent popularity and success as a background context suggest a strong likelihood of overall tour success\footnote{\url{https://chatgpt.com/share/2ed7b17f-322a-4c6d-b22f-268a96463560}}. This choice, however, exemplifies the {\bf conjunction fallacy}. It is logically necessary that the probability of a conjunction of two events (e.g., Taylor Swift's first show is a flop, {\it and} she will eventually sell over a million tickets for the entire tour) is less than the probability of either event alone. 


\textbf{TODO: Maybe it is not necessary to talk about this paragraph. We have clear examples in section 4. Prelim only needs to let readers know what each fallacy is.}

\textbf{TODO: Or should we use the Linda problem as an illustration instead? We have had the example in Figure 2 and it might be more natural to introduce the idea of data perturbation.}
\textbf{TODO:Yeah maybe. I have used this Taylor Swift example in section 4 already. }
However, when the name "Taylor Swift" is changed to a generic name "Nancy", disentangling the semantic narrative that concerts Taylor Swift's current success, LLMs tend to say outcome (a) is more likely than outcome (b).\footnote{\url{https://chatgpt.com/share/46d025c0-f205-4f4a-972a-55d01a04dad1}} Consequently, we assume that LLMs, trained on immersive amounts of human languages, could be misled by the context and prior information, resulting in cognitive logical errors similar to humans. 

\textbf{TODO: Add brief intro to syllogistic fallacy and framing. Could be a single sentence and put detailed examples in appendix.}
\end{comment}

\paragraph{Syllogistic Fallacy} The syllogistic fallacy documents the logical failure that occurs when people are presented with syllogisms -- two premises followed by a conclusion. Ideally, if the premises are true and the logical structure is valid, the conclusion must necessarily be true. However, when the argument's structure is flawed, the conclusion may be invalid despite the surface-level logical form. For example, consider the following syllogism from \citet{kahneman2011thinking}:

\vspace{1mm}
\textit{Is this logically sound?}
\begin{quote}
\vspace{-1mm}
\textit{All roses are flowers.} \\
\textit{Some flowers fade quickly.}\\
\textit{Therefore some roses fade quickly.}
\vspace{-1mm}
\end{quote}

%Both humans and LLMs are likely to endorse this syllogism as valid\footnote{\url{https://chatgpt.com/share/12553aa1-f47b-41bd-a94a-c24ecacb9fe3}}. In fact, the roses could belong to the subgroup of flowers that do not fade quickly so the argument is incorrect \citep{kahneman2011thinking}.

The argument is incorrect because the two premises do not imply that the set of roses and the set of flowers that fade quickly necessarily overlap. 

%The framing problem refers to a cognitive bias where people's decisions are influenced by the way information is presented, rather than just the information itself. This phenomenon demonstrates that the same fact or decision-making scenario can lead to different judgement. The framing effect challenges the notion of human rationality, suggesting that individuals do not always make decisions based on objective reality, but rather on their perception shaped by the presentation of information. We discover that LLMs also fall into such bias. 

